Schema Validation and Evolution for Graph Databases

Despite the maturity of commercial graph databases, little consensus has been reached so far on the standardization of data definition languages (DDLs) for property graphs (PG). The discussion on the characteristics of PG schemas is ongoing in many standardization and community groups. Although some basic aspects of a schema are already present in Neo4j 3.5, like in most commercial graph databases, full support is missing allowing to constraint property graphs with more or less flexibility. In this paper, we focus on two different perspectives from which a PG schema should be considered, as being descriptive or prescriptive, and we show how it would be possible to switch from one to another as the application under development gains more stability. Apart from proposing concise schema DDL inspired by Cypher syntax, we show how schema validation can be enforced through homomorphisms between PG schemas and PG instances; and how schema evolution can be described through the use of graph rewriting operations. Our prototypical implementation demonstrates feasibility and shows the need of offering high-level query primitives to accommodate flexible graph schema requirements as showcased in our work.

==> img/safe_merge_phase_2_p.tex <==
\begin{tikzpicture}[person/.style={draw, circle, fill=red!40!white}, post/.style={draw, circle, fill=blue!40!white}, tmp_post/.style={draw, circle, pattern=custom north west lines, hatchspread=10pt, hatchthickness=3pt, hatchcolor=blue!40!white}, comment/.style={draw, circle, fill=yellow!40!white},  tmp_comment/.style={draw, circle, pattern=custom north west lines, hatchspread=10pt, hatchthickness=3pt, hatchcolor=yellow!40!white},
hybrid/.style={preaction={fill, yellow!40!white}, tmp_post}, attributes/.style={draw},attribute edge/.style={-, black!40!white}, graph edge/.style={-latex}, neutral/.style={draw, circle, fill=black!20!white}]
	\linespread{0.5}
	
	
	% ------------------- P
	\node (p_label) at (-1.25, 3.75) {\color{Orange} $P$};
	\node[scale=0.6] (p) at (0, 3.75) {
		\begin{tikzpicture}
			\node[tmp_post, draw=Orange, line width=1pt, minimum width=0.8cm] (pa) at (0, 4.75) {\large $a$};
	
			\node[tmp_comment, draw=Orange, line width=1pt, minimum width=0.8cm] (pb) at (1.5, 4.75) {\large $b$};	
			
			% edge
			\draw[-latex, Orange, line width=1pt] (pb) edge (pa);
			% -------------------------------------------------
		\end{tikzpicture}
	};
	
	
	%--------------------------- G
	\node (p_label) at (-1.25, 2.25) {\color{Orange} $G$};
	\node (phantom) at (0, 2) {};

	% nodes
	% Bryn|Davies|male|1985-07-03	
	\node[person] (n1) at (0, 0) {\scriptsize $n_1$};
	% \node[draw, minimum width=1.5cm, align=left] (n1_attrs) at (-1.1, -0.85) {\tiny firstName:\ Bryn\\ \tiny lastName:\ Davies};	
	
	\node[post] (n2) at (-1, 1.5) {\scriptsize $n_2$};
	% \node[draw=black!40!white, minimum width=1.5cm, align=left] (n2_attrs) at (-0.65, 2.5) {\tiny imageFile:\ photo33711.jpg \\ \tiny creationDate:\ 2010-10-16\\ \tiny browserUsed:\ Firefox};	
	
	% Jose|Alonso|male|1987-09-18	
	\node[person] (n3) at (1.8, 2.5) {\scriptsize $n_3$};
	% \node[draw=black!40!white, minimum width=1.5cm, align=left] (n3_attrs) at (2, 3.35) {\tiny firstName:\ Jose\\ \tiny lastName:\ Alonso};	
	
	\node[tmp_post, draw=Orange, line width=1pt] (n4) at (2, 0) {\scriptsize $n_4$};
	% \node[draw=black!40!white, minimum width=1.5cm, align=left] (n4_attrs) at (2, -0.85) {\tiny creationDate:\ 2010-10-30\\ \tiny browserUsed:\ Firefox};		
	
	% Jane|Murray|female|1982-09-15|
	\node[person] (n5) at (3.5, 1) {\scriptsize $n_5$};
	% \node[draw=black!40!white, minimum width=1.5cm, align=left] (n5_attrs) at (5.5, 2.15) {\tiny firstName:\ Jane\\ \tiny lastName:\ Murray};		
	
	\node[comment] (n6) at (3.95, 2.5) {\scriptsize $n_6$};
	% \node[draw=black!40!white, minimum width=1.5cm, align=left] (n6_attrs) at (5, 3.35) {\tiny creationDate:\ 2010-10-30\\ \tiny browserUsed:\ Safari};	
	
	\node[tmp_comment, draw=Orange, line width=1pt] (n7) at (6, 0) {\scriptsize $n_7$};
	% \node[draw=black!40!white, minimum width=1.5cm, align=left] (n7_attrs) at (5, -0.85) {\tiny creationDate:\ 2010-10-30\\ \tiny browserUsed:\ Safari};		
	%\node[comment] (n11) at (6, -1) {\scriptsize $n_{11}$};
	
	% attrs to nodes -------
	% \draw[-, black!40!white] (n1_attrs) edge (n1);
	% \draw[-, black!40!white] (n2_attrs) edge (n2);
	% \draw[-, black!40!white] (n3_attrs) edge (n3);
	% \draw[-, black!40!white] (n4_attrs) edge (n4);
	% \draw[-, black!40!white] (n6_attrs) edge (n6);	
	% \draw[-, black!40!white] (n5_attrs.west) edge (n5);	
	% \draw[-, black!40!white] (n7_attrs) edge (n7);	
	
	% edges ------------
	\draw[-latex] (n1) edge node[midway, sloped, fill=white] {\tiny \texttt{LIKES}}  (n2);
	\draw[-latex] (n1) edge[bend right=20] node[midway, sloped, fill=white] {\tiny \texttt{KNOWS}}  (n3);
	\draw[-latex] (n3) edge[bend right=20] node[midway, sloped, fill=white] {\tiny \texttt{KNOWS}}  (n5);
	\draw[-latex] (n1) edge  node[midway, sloped, fill=white] {\tiny \texttt{LIKES}} (n4);
	\draw[-latex] (n2) edge[bend right=20]  node[midway, sloped, fill=white] {\tiny \texttt{HAS\_CREATOR}}  (n3);
	\draw[-latex] (n3) edge node[midway, sloped, fill=white] {\tiny \texttt{LIKES}}   (n4);
	\draw[-latex] (n6) edge  node[midway, sloped, fill=white] {\tiny \texttt{HAS\_CREATOR}} (n3);
	\draw[-latex] (n4) edge  node[above, sloped, fill=white, inner sep=0.5pt, yshift=3pt] {\tiny \texttt{HAS\_CREATOR}} (n5);
	\draw[-latex] (n6) edge[bend right=15] node[midway, sloped, fill=white] {\tiny \texttt{REPLY\_OF}}  (n7);
	\draw[-latex] (n7) edge  node[midway, sloped, fill=white] {\tiny \texttt{HAS\_CREATOR}}  (n5);
	\draw[-latex, Orange, line width=1pt] (n7) edge node[midway, sloped, fill=white] {\tiny \texttt{REPLY\_OF}}  (n4);
	
	% -----------------
	% MATCHING EDGE
	\draw[>->, Orange, line width=0.5pt, shorten <= 0.05cm, shorten >= 0.05cm] (p) edge node[right] {$m$} (phantom);
\end{tikzpicture}

